MARS: Meta-Learning as Score Matching in the Function Space

Meta-learning aims to extract useful inductive biases from a set of related datasets. In Bayesian meta-learning, this is typically achieved by constructing a prior distribution over neural network parameters. However, specifying families of computationally viable prior distributions over the high-dimensional neural network parameters is difficult. As a result, existing approaches resort to meta-learning restrictive diagonal Gaussian priors, severely limiting their expressiveness and performance. To circumvent these issues, we approach meta-learning through the lens of functional Bayesian neural network inference, which views the prior as a stochastic process and performs inference in the function space. Specifically, we view the meta-training tasks as samples from the data-generating process and formalize meta-learning as empirically estimating the law of this stochastic process. Our approach can seamlessly acquire and represent complex prior knowledge by meta-learning the score function of the data-generating process marginals instead of parameter space priors. In a comprehensive benchmark, we demonstrate that our method achieves state-of-the-art performance in terms of predictive accuracy and substantial improvements in the quality of uncertainty estimates.

==> archive.tex <==
\section{Methodology}
\subsection{Choosing the estimator}
\paragraph{Score estimation methods.}
Dealing with intractable probability functions presents one of the key challenges in probabilistic machine learning. A popular approach to this problem is statistical estimation of the log-probability gradient $\nabla_{\mathbf{x}} \log p(\mathbf{x})$, i.e. the \textit{score}. Score estimators can be divided into parametric and nonparametric ones. There are several theoretically-motivated nonparametric score estimation methods that possess well understood properties and straightforward implementations. Their simplicity and flexibility makes them a popular choice \citep{ssgeapplication,fsvgd, steinapplication}. Parametric methods in this area, however, remain relatively scarcely investigated, potentially due to few objectives whose minimization allows for direct parameterization of the score; the most popular being the score matching objective \citep{hyvarinenscorematching}, i.e., the expected squared
distance between the gradient of the log-density given by the model and the gradient of
the log-density of the observed data. Another approach to direct parameterization of the score can be established by minimization of the  DEEN objective \citep{deen}, however this has been shown not to be robust and result in poor performance \citep{alainbengio}. Both parametric and nonparametric methods rely on availability of large amount of data, otherwise resulting in scores of non-smooth, overconfident distributions (see Figures \ref{badssgenu}, \ref{badandgood}).



\begin{table}
  \caption{Cosine similarity between the predicted and true score of a $d$-dimensional Gaussian}
  \label{nonparamcomparison}
  \centering
  \begin{tabular}{lllll}
    \toprule
    Estimator     & $d=2$     & $d=5$   & $d=10$  & $d=15$  \\
    \midrule
    KEF                 &  0.8510 $\pm$   0.0272  & 0.8333 $\pm$ 0.0178      & 0.1207 $\pm$  0.0091      & 0.0733 $\pm$  0.0172      \\
    Tikhonov + Nyström  &  0.5322 $\pm$   0.0387  & 0.8051 $\pm$ 0.0363      & 0.0939 $\pm$   0.0077      & 0.0498 $\pm$  0.0087       \\
   Landweber iter.      &  0.9413 $\pm$  0.0121  & 0.2456 $\pm$ 0.0170      & 0.0385 $\pm$  0.0010      & 0.0135 $\pm$  0.0047     \\
   $\nu$-method         &  0.6741 $\pm$  0.0326  & 0.8132 $\pm$ 0.0427      & 0.1513 $\pm$  0.0087      & 0.0876 $\pm$  0.0022      \\
  SSGE w. $\eta=0.0001$ &  \textbf{0.9673 $\pm$   0.0119}  & 0.3329 $\pm$ 0.0278      & 0.0455 $\pm$  0.0064      & 0.0422 $\pm$  0.0019      \\
      \textsc{ARSEN} (Our)       & \textbf{0.9679} $\pm$ \textbf{0.0147} & \textbf{0.9359} $\pm$ \textbf{0.0251} & \textbf{0.3195} $\pm$ \textbf{0.0512} & \textbf{0.2011} $\pm$ \textbf{0.0166}\\
    \bottomrule
  \end{tabular}
\end{table}




\paragraph{Nonparametric score estimation.}
There is a plethora of nonparametric score estimation methods; KEF \citep{kef} minimizes a regularized version of the score matching loss between the data score and score of kernel exponential families. NKEF  \citep{nkef} relies on the Nyström method to accelerate KEF by minimizing the loss in a low-dimensional subspace, rather than the whole RKHS. \citet{stein} utilize the generalized Stein's identity to propose the Stein estimator, and \citet{ssge} propose Spectral Stein Gradient Estimator (SSGE) by expanding the score function in terms of the spectral eigenbasis. Together with iterative methods ($\nu$-method and Landweber iteration \citep{numethod}), these can be naturally unified through a regularized, nonparametric regression framework \citep{nonparametric}. However, nonparametric estimators present two problems: none of the estimators provide a principled way to reason about stochastic process scores and in the low-data regime, they result in scores of overconfident distributions, non-smooth distributions.

\paragraph{Score matching and parametric estimators.} Parametric objectives, as they are expectations, require Monte Carlo estimation and rely heavily on abundance of data in order to result in solid performance. These objectives have seen a large popularity in the field of GANs \citep{gans} where the data assumption is commonly satisfied. Furthermore, due to the high dimensionality of the input/output domain, the subsequent research on the objectives mainly focused on the low-dimensional approximations \citep{slicedscorematching, slicedscorematching2}. However, regularization in the low-data regime remains poorly understood. 
\paragraph{The final choice.} Although neither methods present a well-explored regularization method, parametric methods present a better choice, for the following reasons. Parameterizing the score using a neural network introduces a vast toolset of smoothing method which can be empirically explored. Furthermore, there is a straightforward way of reasoning about the whole stochastic process, rather than distributions: by concatenating the measurement points with their functional evaluations and inputting this to the neural network, we can use the score matching loss to infer about the stochastic process directly. We explain this next.


\subsection{Learning the stochastic process}
In this work, we propose \textsc{ARSEN}, a parametric framework that uses self-attention in order to capture similarities between functional evaluations and learn the score of marginal distributions of some underlying stochastic process. Self-attention was first proposed by \citet{vaswani2017attention} within the concept of Transformers, neural network architectures that effectively learn dependencies between inputs, particularly between distant inputs in a sentence/text. \textit{Self-Attention}, as a key ingredient of the Transformer architecture allows relating different positions of a sequence in order to compute a representation of the sequence. One important property of attention is that, if positional encodings are not used, it makes the network permutation equivariant w.r.t. its inputs, as observed in \citep{settransformer}. 

In order to maximize sample efficiency, we impose an architecture satisfying the equivariance properties of gradient functions: by self-attending without positional embeddings, we achieve permutation equivariance across the sample dimension \citep{settransformer}. Furthermore, in order to capture the positional relationships between functional evaluations of different inputs, we propose using the input embeddings as queries and keys, whereas the functional evaluations ones are used as values. This is shown in Figure \ref{arsen}. The architecture details are provided in Appendix.

\subsection{Preventing meta-overfitting}
In order to tackle overfitting, we gather inspiration from GAN stabilization techniques. More specifically, we consider: \emph{(i)} gradient penalties \citep{gradientpenalty}, where gradient evaluations of points uniformly sampled on a linear interpolation between the data are added as a soft penalty and \emph{(ii)} spectrally normalizing the network's linear layers \citep{spectralnormalization}. We also experiment with the following soft penalties: \emph{(iii)} sum of spectrals norm of linear layers, and \emph{(iv)} adding the RKHS norm w.r.t. a curl-free kernel.\footnote{Note that every gradient function has a curl-free kernel, therefore the network should have a finite RKHS norm w.r.t. a curl-free kernel.} 

We find spectral normalization of linear layers to perform best. In order to compare naively fitting the proposed network (no regularization) and spectral normalization, we we use Random Fourier Features \citep{rff} and sample 10 functions from a GP with an radial basis function kernel. We train both network on $5$-dimensional samples from the distribution by uniformly sampling inputs from $[-7,7]^5$. The network is provided noisy function evaluations, with a Gaussian $N(0,0.1^2)$ noise. In INSERTREFHERE, we present the comparison showcasing that the proposed regularization successfully hinders overfitting, and in Figure INSERTREFHERE, we provide evidence that the regularization does not hinder flexibility and approximation capability of the network. Finally, we compare the performance of our network with nonparametric estimators on distributional estimation; we sample only from one distribution, induced by fixed measurement points. We find out method to significantly outperform all nonparametric score estimation methods.

\subsection{Incorporating uncertainty about scarcity in the x-domain}
As another precaution against meta-overfitting we propose the following. Assume we have access to $m_i$ evaluations of functions $f_i$, $i=1,...,n$ at possibly different inputs. In order to capture uncertainty about scarcity in the input domain, we propose fitting a GP to each of the functions $f_i$ and training \textsc{ARSEN} on the samples from these GPs. An example of this is given in Figure \ref{sumpic}, where we train the ARSEN network on 10 noised functions evaluated at 5 uniformly sampled input from $[-5,-2]\cup[2,5]$. We can see the difference between training ARSEN with and without the GP interpolation: the network yields much larger uncertainty between $x=-2$ and $x=2$ as the GP interpolation resulted in learning the scores of much wider distributions. In our experiments, we use the Matérn kernel with $\nu=5/2$ as a universal kernel\citep{micchelli2006universal} (i.e., \textit{cc-}universal \citep{ccuniversal})) and use cross-validation to select the length scale and variance parameter. However, one can easily control for the prudence of the model by controlling the kernel parameters.

==> iclr2023/archive.tex <==
\section{Methodology}
\subsection{Choosing the estimator}
\paragraph{Score estimation methods.}
Dealing with intractable probability functions presents one of the key challenges in probabilistic machine learning. A popular approach to this problem is statistical estimation of the log-probability gradient $\nabla_{\mathbf{x}} \log p(\mathbf{x})$, i.e. the \textit{score}. Score estimators can be divided into parametric and nonparametric ones. There are several theoretically-motivated nonparametric score estimation methods that possess well understood properties and straightforward implementations. Their simplicity and flexibility makes them a popular choice \citep{ssgeapplication,fsvgd, steinapplication}. Parametric methods in this area, however, remain relatively scarcely investigated, potentially due to few objectives whose minimization allows for direct parameterization of the score; the most popular being the score matching objective \citep{hyvarinenscorematching}, i.e., the expected squared
distance between the gradient of the log-density given by the model and the gradient of
the log-density of the observed data. Another approach to direct parameterization of the score can be established by minimization of the  DEEN objective \citep{deen}, however this has been shown not to be robust and result in poor performance \citep{alainbengio}. Both parametric and nonparametric methods rely on availability of large amount of data, otherwise resulting in scores of non-smooth, overconfident distributions (see Figures \ref{badssgenu}, \ref{badandgood}).



\begin{table}
  \caption{Cosine similarity between the predicted and true score of a $d$-dimensional Gaussian}
  \label{nonparamcomparison}
  \centering
  \begin{tabular}{lllll}
    \toprule
    Estimator     & $d=2$     & $d=5$   & $d=10$  & $d=15$  \\
    \midrule
    KEF                 &  0.8510 $\pm$   0.0272  & 0.8333 $\pm$ 0.0178      & 0.1207 $\pm$  0.0091      & 0.0733 $\pm$  0.0172      \\
    Tikhonov + Nyström  &  0.5322 $\pm$   0.0387  & 0.8051 $\pm$ 0.0363      & 0.0939 $\pm$   0.0077      & 0.0498 $\pm$  0.0087       \\
   Landweber iter.      &  0.9413 $\pm$  0.0121  & 0.2456 $\pm$ 0.0170      & 0.0385 $\pm$  0.0010      & 0.0135 $\pm$  0.0047     \\
   $\nu$-method         &  0.6741 $\pm$  0.0326  & 0.8132 $\pm$ 0.0427      & 0.1513 $\pm$  0.0087      & 0.0876 $\pm$  0.0022      \\
  SSGE w. $\eta=0.0001$ &  \textbf{0.9673 $\pm$   0.0119}  & 0.3329 $\pm$ 0.0278      & 0.0455 $\pm$  0.0064      & 0.0422 $\pm$  0.0019      \\
      \textsc{ARSEN} (Our)       & \textbf{0.9679} $\pm$ \textbf{0.0147} & \textbf{0.9359} $\pm$ \textbf{0.0251} & \textbf{0.3195} $\pm$ \textbf{0.0512} & \textbf{0.2011} $\pm$ \textbf{0.0166}\\
    \bottomrule
  \end{tabular}
\end{table}




\paragraph{Nonparametric score estimation.}
There is a plethora of nonparametric score estimation methods; KEF \citep{kef} minimizes a regularized version of the score matching loss between the data score and score of kernel exponential families. NKEF  \citep{nkef} relies on the Nyström method to accelerate KEF by minimizing the loss in a low-dimensional subspace, rather than the whole RKHS. \citet{stein} utilize the generalized Stein's identity to propose the Stein estimator, and \citet{ssge} propose Spectral Stein Gradient Estimator (SSGE) by expanding the score function in terms of the spectral eigenbasis. Together with iterative methods ($\nu$-method and Landweber iteration \citep{numethod}), these can be naturally unified through a regularized, nonparametric regression framework \citep{nonparametric}. However, nonparametric estimators present two problems: none of the estimators provide a principled way to reason about stochastic process scores and in the low-data regime, they result in scores of overconfident distributions, non-smooth distributions.

\paragraph{Score matching and parametric estimators.} Parametric objectives, as they are expectations, require Monte Carlo estimation and rely heavily on abundance of data in order to result in solid performance. These objectives have seen a large popularity in the field of GANs \citep{gans} where the data assumption is commonly satisfied. Furthermore, due to the high dimensionality of the input/output domain, the subsequent research on the objectives mainly focused on the low-dimensional approximations \citep{slicedscorematching, slicedscorematching2}. However, regularization in the low-data regime remains poorly understood. 
\paragraph{The final choice.} Although neither methods present a well-explored regularization method, parametric methods present a better choice, for the following reasons. Parameterizing the score using a neural network introduces a vast toolset of smoothing method which can be empirically explored. Furthermore, there is a straightforward way of reasoning about the whole stochastic process, rather than distributions: by concatenating the measurement points with their functional evaluations and inputting this to the neural network, we can use the score matching loss to infer about the stochastic process directly. We explain this next.


\subsection{Learning the stochastic process}
In this work, we propose \textsc{ARSEN}, a parametric framework that uses self-attention in order to capture similarities between functional evaluations and learn the score of marginal distributions of some underlying stochastic process. Self-attention was first proposed by \citet{vaswani2017attention} within the concept of Transformers, neural network architectures that effectively learn dependencies between inputs, particularly between distant inputs in a sentence/text. \textit{Self-Attention}, as a key ingredient of the Transformer architecture allows relating different positions of a sequence in order to compute a representation of the sequence. One important property of attention is that, if positional encodings are not used, it makes the network permutation equivariant w.r.t. its inputs, as observed in \citep{settransformer}. 

In order to maximize sample efficiency, we impose an architecture satisfying the equivariance properties of gradient functions: by self-attending without positional embeddings, we achieve permutation equivariance across the sample dimension \citep{settransformer}. Furthermore, in order to capture the positional relationships between functional evaluations of different inputs, we propose using the input embeddings as queries and keys, whereas the functional evaluations ones are used as values. This is shown in Figure \ref{arsen}. The architecture details are provided in Appendix.

\subsection{Preventing meta-overfitting}
In order to tackle overfitting, we gather inspiration from GAN stabilization techniques. More specifically, we consider: \emph{(i)} gradient penalties \citep{gradientpenalty}, where gradient evaluations of points uniformly sampled on a linear interpolation between the data are added as a soft penalty and \emph{(ii)} spectrally normalizing the network's linear layers \citep{spectralnormalization}. We also experiment with the following soft penalties: \emph{(iii)} sum of spectrals norm of linear layers, and \emph{(iv)} adding the RKHS norm w.r.t. a curl-free kernel.\footnote{Note that every gradient function has a curl-free kernel, therefore the network should have a finite RKHS norm w.r.t. a curl-free kernel.} 

We find spectral normalization of linear layers to perform best. In order to compare naively fitting the proposed network (no regularization) and spectral normalization, we we use Random Fourier Features \citep{rff} and sample 10 functions from a GP with an radial basis function kernel. We train both network on $5$-dimensional samples from the distribution by uniformly sampling inputs from $[-7,7]^5$. The network is provided noisy function evaluations, with a Gaussian $N(0,0.1^2)$ noise. In INSERTREFHERE, we present the comparison showcasing that the proposed regularization successfully hinders overfitting, and in Figure INSERTREFHERE, we provide evidence that the regularization does not hinder flexibility and approximation capability of the network. Finally, we compare the performance of our network with nonparametric estimators on distributional estimation; we sample only from one distribution, induced by fixed measurement points. We find out method to significantly outperform all nonparametric score estimation methods.

\subsection{Incorporating uncertainty about scarcity in the x-domain}
As another precaution against meta-overfitting we propose the following. Assume we have access to $m_i$ evaluations of functions $f_i$, $i=1,...,n$ at possibly different inputs. In order to capture uncertainty about scarcity in the input domain, we propose fitting a GP to each of the functions $f_i$ and training \textsc{ARSEN} on the samples from these GPs. An example of this is given in Figure \ref{sumpic}, where we train the ARSEN network on 10 noised functions evaluated at 5 uniformly sampled input from $[-5,-2]\cup[2,5]$. We can see the difference between training ARSEN with and without the GP interpolation: the network yields much larger uncertainty between $x=-2$ and $x=2$ as the GP interpolation resulted in learning the scores of much wider distributions. In our experiments, we use the Matérn kernel with $\nu=5/2$ as a universal kernel\citep{micchelli2006universal} (i.e., \textit{cc-}universal \citep{ccuniversal})) and use cross-validation to select the length scale and variance parameter. However, one can easily control for the prudence of the model by controlling the kernel parameters.

==> iclr2023/content/abstract.tex <==
\begin{abstract}
\vspace{-6pt}
\looseness -1 
Meta-learning aims to extract useful inductive biases from a set of related datasets. In Bayesian meta-learning, this is typically achieved by constructing a prior distribution over neural network parameters. However, specifying families of computationally viable prior distributions over the high-dimensional neural network parameters is difficult. As a result, existing approaches resort to meta-learning restrictive diagonal Gaussian priors, severely limiting their expressiveness and performance. To circumvent these issues, we approach meta-learning through the lens of functional Bayesian neural network inference, which views the prior as a stochastic process and performs inference in the function space. Specifically, we view the meta-training tasks as samples from the data-generating process and formalize meta-learning as empirically estimating the law of this stochastic process. Our approach can seamlessly acquire and represent complex prior knowledge by meta-learning the score function of the data-generating process marginals instead of parameter space priors. In a comprehensive benchmark, we demonstrate that our method achieves state-of-the-art performance in terms of predictive accuracy and substantial improvements in the quality of uncertainty estimates.
% %In our experiments, we demonstrate that {\em MARS} can express complex inductive biases seamlessly 
% In a comprehensive benchmark study, we demonstrate that MARS



% %, called {\em Meta-learning via Attention-based Regularised Score estimation (MARS)}. 



% In particular, we propose to meta-learn the {\em score} of its the marginal distributions, which can then directly be used as source of prior knowledge when we perform functional approximate BNN inference






% OLD ABSTRACT (IGNORE):
% Meta-learning provides a powerful tool for extracting knowledge about the underlying data generation process. In order to tackle meta-data scarcity and prevent meta-overfitting, researchers gained strong interest in estimating uncertainty. Although Bayesian deep learning (BDL) provides plethora of uncertainty estimation methods, these often make very stringent assumptions which hinder their integration with meta-learning. To alleviate the challenges of integrating BDL with meta-learning, we propose a novel algorithm that propagates the extracted knowledge through a functional-prior score estimator network, that is used to directly enhance Bayesian neural network (BNN) training. We provide empirical evidence that our proposed architecture prevents meta-overfitting and works well in the low data regime. We further show that, while achieving state-of-the-art score estimation performance, the regularized network successfully incorporates meta-learned knowledge into the BNN. Our method significantly outperforms several other meta-learning algorithms, both in terms of predictive accuracy and uncertainty calibration on several datasets.
\end{abstract}

==> iclr2023/content/background.tex <==
\vspacecaption
\section{Background}
\vspacecaptionlow
\label{sec:background}

% \looseness -1 We briefly review the basics of BNNs and describe how to view BNN inference from a function space perspective.
%, introducing the notation that the remainder of the paper draws upon.

\textbf{Bayesian Neural Networks. }
Consider a regression task with data $\mathcal{D}=\left(\mathbf{X}^{\mathcal{D}},\mathbf{y}^{\mathcal{D}}\right)$ that consists of $m$ i.i.d.\ noisy function evaluations
$y_{j}=f\left(\bx_{j}\right)+ \epsilon_j$ of an unknown function $f: \calX \mapsto \calY$. 
Here, $\mathbf{X}^{\mathcal{D}} = \left\{ \bx_j \right\}_{j=1}^m \in \calX^m$ denotes training inputs and $\mathbf{y}^{\mathcal{D}} = \left\{ y_j \right\}_{j=1}^m \in \calY^m$ the corresponding noisy function values.
Let $h_\theta: \calX \rightarrow \calY$ be a function parametrized by a NN with weights $\theta \in \Theta$. For regression, 
%For real-valued regression 
where $\calY \subseteq \R$, we can use $h_\theta$ to define a conditional distribution over the noisy observations $p(y|\bx,\theta) = \calN(y|h_\theta(\bx), \sigma^2)$, with flexible mean represented by $h_\theta$ and observation noise variance $\sigma^2$. 
%For Bayesian inference, one presumes a 
Given a prior distribution $p(\theta)$ over the model parameters $\theta$, %together with the training data $\mathcal{D}$, 
Bayes' theorem
%which is combined with  $\mathcal{D}$ into a
yields a posterior distribution $p(\theta|\mathbf{X}^{\mathcal{D}}, \mathbf{y}^{\mathcal{D}}) \propto p(\mathbf{y}^{\mathcal{D}}|\mathbf{X}^{\mathcal{D}},\theta) p(\theta)$,
where $p(\mathbf{y}^{\mathcal{D}}|\mathbf{X}^{\mathcal{D}},\theta) = \prod_{j=1}^m p(y_j | \mathbf{x}_j, \theta)$. For an unseen test point $\bx^*$, we compute the predictive distribution, which is defined as $p(y^*|\bx^*,\mathbf{X}^{\mathcal{D}}, \mathbf{y}^{\mathcal{D}}) = \int p(y^*|\bx^*,\theta) p(\theta|\mathbf{X}^{\mathcal{D}}, \mathbf{y}^{\mathcal{D}}) d\theta$ and obtained by marginalizing out the posterior over parameters $\theta$.

\textbf{BNN inference in the function space. }
%
\looseness -1 Posterior inference for BNNs is difficult due to the high-dimensional parameter space $\Theta$ and the over-parameterized nature of the NN mapping $h_\theta(x)$. 
An alternative approach views BNN inference in the function space, i.e., the space of regression functions $h: \calX \mapsto \calY$, yielding the Bayes rule $p(h |\mathbf{X}^{\mathcal{D}}, \mathbf{y}^{\mathcal{D}}) \propto p(\mathbf{y}^{\mathcal{D}} | \mathbf{X}^{\mathcal{D}},h) p(h)$ \citep{wang2019function, sun2019}. Here, $p(h)$ is a stochastic process prior with index set $\calX$, taking values in $\calY$. 
%Since there exists a (differentiable) map $\psi: \theta \mapsto h_\theta(\cdot)$ from the neural network weights $\theta$ to its corresponding regression function $h$, we can maintain a variational distribution or particle approximation of the posterior in the weight space. 
%Given any distribution $q(\theta)$ on network parameters, we can use $\psi$ to obtain its pushforward measure in the function space. 

\looseness -1 Stochastic processes can be understood as infinite-dimensional random vectors, and, thus, are hard to work with computationally. However, 
given finite measurement sets $\mathbf{X} := [\bx_1, ..., \bx_k] \in \calX^k, k \in \mathbb{N}$, the stochastic process can be characterized by its corresponding marginal distributions of function values $\rho(\mathbf{h}^\mathbf{X}):= \rho(h(\bx_1), ... h(\bx_k))$ (cf. Kolmogorov Extension Theorem, \citet{stochastic_differential_equations}).  Thus, we can break down the functional posterior into a more tractable form by re-phrasing it in terms of posterior marginals based on measurement sets $\bX$:
$p(\rvh^\bX |\mathbf{X}, \mathbf{X}^\mathcal{D}, \mathbf{y}^{\mathcal{D}})  \propto  p(\mathbf{y}^{\mathcal{D}} | \rvh^{\bX^{\mathcal{D}}}) p(\rvh^{\bX})$. 

\looseness -1 This functional posterior can be tractably approximated to achieve functional BNN inference \citep{sun2019, wang2019function}. 
We briefly describe how this can be done via functional Stein Variational Gradient Descent  \citep[fSVGD,][]{wang2019function}. The procedure is explained in more detail in Appendix~\ref{appx:fsvgd_detail}.
The fSVGD algorithm approximates the posterior using a set of $L$ NN parameter particles $\{ \theta_1, ..., \theta_L \}$. To optimize posterior approximation, fSVGD iteratively re-samples measurement sets $\bX$ from a measurement distribution $\nu$, supported on $\calX$, computes SVGD updates \citep{Liu2016} in the function space, and projects them back into the parameter space, in order to update the parameter-space particle configuration approximating the posterior. 
%
To achieve this, fSVGD uses the functional posterior score, i.e., the gradient of the log-density
$\nabla_{\rvh^\bX} \ln p(\rvh^\bX |\mathbf{X},  \mathbf{X}^\mathcal{D},\mathbf{y}^{\mathcal{D}})  = \nabla_{\rvh^\bX} \ln p(\mathbf{y}^{\mathcal{D}} | \rvh^{\bX^{\mathcal{D}}}) + \nabla_{\rvh^\bX} \ln p(\rvh^{\bX})$ to guide the particles towards areas of high posterior probability. Formally, for all $l = 1, ..., L~$ the particle updates are computed as
%
\begin{equation} \label{eq:fsvgd_updates}
% \resizebox{0.91\hsize}{!}{
%     $
    \theta^l \leftarrow \theta^l - \gamma  \left( \nabla_{\theta^l} \rvh_{\theta^l}^\bX \right)^\top  \bigg( \underbrace{\frac{1}{L} \sum_{i=1}^L \bK_{li} \nabla_{\rvh_{\theta^i}^\bX} \ln p(\rvh_{\theta^l}^\bX |\mathbf{X}, \mathbf{X}^\mathcal{D}, \mathbf{y}^{\mathcal{D}}) + \nabla_{\rvh_{\theta^l}^\bX} \bK_{li}}_{\text{SVGD update in the function space} \vspace{-4pt}} \bigg) ~ \;
    % $
    % }
\end{equation}
where $\mathbf{K} = [k(\rvh_{\theta^l}^\bX, \rvh_{\theta^i}^\bX)]_{li}$ is the kernel matrix between the function values in the measurement points based on a positive semi-definite kernel function $k(\cdot, \cdot)$. A key insight that will later draw upon in the paper is that such functional approximate inference techniques only use the prior scores and, in principle, do not require a full prior density that integrates to 1.

%When we perform posterior inference with the meta-learned score network, we simply replace the hand-defined prior score $\nabla_{\rvh^\bX} \ln p(\rvh^{\bX})$ with the predictions meta-learned score network $s(\rvh_{\theta^l}^\bX, \bX)$.


==> iclr2023/content/conclusion.tex <==
\vspacecaption
\section{Conclusion}
\vspacecaptionlow
We have introduced a novel meta-learning approach in the function space that estimates the score of the data-generating process marginals from a set of related datasets. When facing a new learning task, we use the meta-learned score network as a source of prior for functional approximate BNN inference.
%
By representing inductive bias as the score of a stochastic process, our approach is versatile and can seamlessly acquire/represent complex prior knowledge. Empirically, this translates into strong performance when compared to previous meta-learning methods. The substantial improvements of \ours in terms of the quality of uncertainty estimates open up many potential extensions toward interactive machine learning where exploration based on epistemic uncertainty is vital.

%While this paper focuses on regression problems; it remains an open problem how to apply our meta-learning approach in the function space to other machine-learning problems such as classification. Additionally, it remains unclear how well our approach in the function space scales to higher-dimensional data domains, as the measurement sets become increasingly sparse in $\calX$.

==> iclr2023/content/experiments.tex <==
\vspacecaption
\section{Experiments}
\vspacecaptionlow
\label{sec:experiments}
% Now that we have a framework that can incorporate uncertainty in the input domain and regularize against overfitting in the output domain, we empirically evaluate the incorporation of ARSEN with fSVGD. We compare the method several other probabilistic meta-learning approaches, demonstrating that: \emph{(i)} we outperform other algorithms in terms of \textit{predictive accuracy}, \emph{(ii)} improve \textit{uncertainty estimation} of probabilistic meta-learning, and \emph{(iii)} successfully prevent for \textit{meta-overfitting}.
%We now empirically examine the implications of our approach. 
We provide a detailed benchmark comparison with existing meta-learning methods, demonstrating
%\footnote{The source code for MARS is available at \href{https://github.com/krunolp/mars}{\texttt{https://github.com/krunolp/mars}}.}
that \ours: \emph{(i)} achieves state-of-the-art performance in terms of predictive accuracy, \emph{(ii)} yields well-calibrated uncertainty estimates. In a comprehensive ablation study, we shed more light on the central components of \ours and provide empirical support for our design decisions.

\begin{figure}
\vspace{-5pt}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \vspace{-3pt}
         \includegraphics[width=\linewidth, trim= 0 30 0 0, clip]{iclr2023/images/fig_2_a.pdf}
         \vspace{-13pt}
         \caption{Vanilla BNN}
         \label{plt1bad}
     \end{subfigure}
     \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
          \vspace{-3pt}
         \includegraphics[width=\linewidth,  trim= 0 30 0 0, clip]{iclr2023/images/fig_2_b.pdf}
         \vspace{-13pt}
         \caption{fBNN with GP prior}
         \label{plt2bad}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
     \centering
      \vspace{-3pt}
     \includegraphics[width=\linewidth,  trim= 0 30 0 0, clip]{iclr2023/images/fig_2_c.pdf}
     \vspace{-13pt}
     \caption{\ours (ours)}
     \label{plt1good}
    \end{subfigure}
    \vspace{-6pt}
  \caption{BNN posterior predictions with (a) zero-centered Gaussian prior on the NN parameters $\theta$ (b) Gaussian process prior and (c) meta-learned MARS prior scores. \vspace{-8pt}}
  \label{fig:posterior_predictions}
\end{figure}

\vspacesubcaption
\subsection{Experiment Setup}
\vspacesubcaptionlow
\label{sec:exp_setup}

%\looseness -1
\textbf{Environments. } We consider five realistic meta-learning environments for \textit{regression}. The first environment corresponds to data of different calibration sessions of the Swiss Free Electron Laser (\emph{SwissFEL}) \citep{milne2017swissfel}. Here, a task requires predicting the laser's beam intensity based on undulators parameters. We also consider electronic health measurements (\emph{PhysioNet}) from intensive care patients \citep{silva2012predicting}, in particular, the Glasgow Coma Scale (\emph{GCS}) and the hematocrit value (\emph{HCT}). Here, each task correspond to a patient. We also use the Intel Berkeley Lab temperature sensor dataset (\emph{Berkeley-Sensor}) \citep{intel_sensor_data}, requiring auto-regressive prediction of temperature measurements of sensors in different locations of the building. Finally, the \emph{Argus-Control} environment requires predicting the total variation of a robot from its target position based on its PID controller parameters \citep{rothfuss2022_safe}. Here, tasks correspond to different step sizes between the source and target location. See Appendix \ref{appendix:meta-envs} for details.

\looseness -1 \textbf{Baselines.}
As non-meta-learning baselines, we use a \emph{Vanilla GP} with RBF kernel and a \emph{Vanilla BNN} with a zero-mean, spherical Gaussian prior and SVGD inference \citep{Liu2016}.
To compare to previous meta-learners, we report results for model agnostic meta-learning (\textit{MAML}) \citep{finn2017model}, Bayesian MAML (\textit{BMAML}) \citep{bmaml} and neural processes (\textit{NPs}) \citep{garnelo2018neural}. In addition, we include {\em PACOH} \citep{rothfuss2021pacoh} which performs hierarchical Bayes inference to meta-learn a GP prior ({\em PACOH-GP}) or prior over NN parameters ({\em PACOH-NN}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspacesubcaption
\subsection{Empirical Benchmark Study}
\vspacesubcaptionlow

\begin{table}
  \centering
  \resizebox{0.9 \textwidth}{!}{
  \begin{tabular}{l|ccccc}
    \toprule
         & SwissFEL   & Physionet-GCS  & Physionet-HCT  & Berkeley-Sensor & Argus-Control \\
    \midrule
    Vanilla GP  &  0.876 $\pm$ 0.000      & 2.240 $\pm$  0.000      & 2.768 $\pm$  0.000     & 0.258 $\pm$ 0.000 & 0.026 $\pm$ 0.000 \\
    Vanilla BNN &  0.529 $\pm$ 0.022      & 2.664 $\pm$  0.274      & 3.938 $\pm$  0.869     & 0.151 $\pm$ 0.018 & 0.016 $\pm$ 0.002 \\ %\hline
    MAML        &  0.730 $\pm$ 0.057      & 1.895 $\pm$  0.141      & 2.413 $\pm$  0.113     & \textbf{0.121} $\pm$ \textbf{0.027} & 0.017 $\pm$ 0.001 \\
    BMAML       &  0.577 $\pm$ 0.044      & 1.894 $\pm$  0.062      & 2.500 $\pm$  0.002    & 0.222 $\pm$ 0.032 & 0.037 $\pm$ 0.003\\
    NP          &  0.471 $\pm$ 0.053      & 2.056 $\pm$  0.209      & 2.594 $\pm$  0.107    &  0.173 $\pm$ 0.018 & 0.020 $\pm$ 0.001\\
    %MLAP        &  0.486 $\pm$ 0.026      & 2.009 $\pm$  0.248      & 2.470 $\pm$  0.039     & 0.348 $\pm$ 0.034 & 0.030 $\pm$ 0.003 \\
    PACOH-GP    &  \textbf{0.376 $\pm$ 0.024}   & \textbf{1.498 $\pm$  0.081}   & 2.361 $\pm$  0.047   & 0.197 $\pm$ 0.058 &  0.016 $\pm$ 0.005 \\
    PACOH-NN    &  0.437 $\pm$ 0.021     & 1.623 $\pm$  0.057      & 2.405 $\pm$  0.017   & 0.160 $\pm$ 0.070 & 0.018 $\pm$ 0.002\\
    \ours-GP (ours) & \textbf{0.391} $\pm$ \textbf{0.011} & \textbf{1.471} $\pm$ \textbf{0.083} & \textbf{2.309} $\pm$ \textbf{0.041} & \textbf{0.116} $\pm$ \textbf{0.024} & \textbf{0.013} $\pm$ \textbf{0.001}\\
    \ours-BNN (ours) & 0.407 $\pm$ 0.061 & \textbf{1.307 $\pm$ 0.065} & 2.248 $\pm$ 0.057 & \textbf{0.113 $\pm$ 0.015} & 0.017 $\pm$ 0.003 
     \\ \bottomrule
    \end{tabular}}
    \vspace{-4pt}
    \caption{Meta-Learning benchmark results in terms of the test RMSE. Reported are the mean and standard deviation across five seeds. \ours consistently yields the most accurate predictions. \vspace{-10pt}}
  \label{meta_learning_mse}
\end{table}

\begin{table}[t]
  \centering
  \resizebox{0.95 \textwidth}{!}{\
  \begin{tabular}{l|ccccc}
    \toprule
         & SwissFEL   & Physionet-GCS  & Physionet-HCT  & Berkeley-Sensor & Argus-Control\\
    \midrule
    Vanilla GP  &  0.135 $\pm$ 0.000      & 0.268 $\pm$  0.000      & 0.277 $\pm$  0.000    &   0.119 $\pm$ 0.000 & 0.090 $\pm$ 0.000\\
    Vanilla BNN &  0.085 $\pm$ 0.008      & 0.277 $\pm$  0.013      & 0.307 $\pm$  0.009    &   0.206 $\pm$ 0.025 & 0.104 $\pm$ 0.005\\
    BMAML        &  0.115 $\pm$ 0.036      & 0.279 $\pm$  0.010      & 0.423 $\pm$  0.106    &   0.154 $\pm$ 0.021 & 0.068 $\pm$ 0.005 \\
    NP       &  0.131 $\pm$ 0.056      & 0.299 $\pm$  0.012      & 0.319 $\pm$  0.004    &   0.140 $\pm$ 0.035 & 0.094 $\pm$ 0.015 \\
    %MLAP        &  0.090 $\pm$ 0.021      & 0.343 $\pm$  0.017      & 0.344 $\pm$  0.016     &  0.183 $\pm$ 0.017 & 0.168 $\pm$ 0.009\\
    PACOH-GP     &  \textbf{0.038 $\pm$ 0.006}      & \textbf{0.262 $\pm$  0.004}      & 0.296 $\pm$  0.003    &   0.251  $\pm$ 0.035 & 0.102 $\pm$ 0.010 \\
    PACOH-NN     &  \textbf{0.037} $\pm$ \textbf{0.005}      & \textbf{0.267} $\pm$  \textbf{0.005}      & 0.302 $\pm$  0.003    &    0.223 $\pm$ 0.012 & 0.119 $\pm$ 0.005 \\
    \ours-GP (ours) & \textbf{0.035} $\pm$ \textbf{0.002} & \textbf{0.263} $\pm$ \textbf{0.001} & \textbf{0.136} $\pm$ \textbf{0.007} & \textbf{0.080} $\pm$ \textbf{0.005} & \textbf{0.055} $\pm$ \textbf{0.002} \\
    \ours-BNN (ours) & 0.054 $\pm$ 0.009 & \textbf{0.268} $\pm$ \textbf{0.023} & 0.231 $\pm$ 0.029 & \textbf{0.078} $\pm$ \textbf{0.020} & 0.076 $\pm$ 0.031 \\
    \bottomrule
  \end{tabular}}
  \vspace{-4pt}
    \caption{Meta-learning benchmark results in terms of the calibration error. Reported are the mean and standard deviation across five seeds. \ours provides the best-calibrated uncertainty estimates.   \vspace{-6pt}}
  \label{meta_learning_ece}
\end{table}

\looseness -1 \textbf{Qualitative illustration. } Fig. \ref{fig:posterior_predictions} illustrates the posterior predictions of a) a BNN with Gaussian Prior in the parameter space, b) a functional BNN with GP prior \citep{wang2019function} and c) a fBNN trained with the meta-learned MARS-GP marginal scores.
For the meta-training we use $n=20$ tasks with each $m=8$ data points, generated from a student-t process with sinusoidal mean function $2x + 5 \sin(2x)$.
%
Similar to previous work \citep[e.g.,][]{fortuin2021bayesian} we observe that weight-space BNN priors provide poor inductive bias and yield grossly over-confident uncertainty estimates. Approaching the BNN inference problem in the function space (see Fig \ref{plt2bad}) results in much better uncertainty estimates. In this case, however, the uninformative GP prior does not result in accurate mean predictions. Finally, the meta-learned scores in the function space provide useful inductive biased towards the linear+sinusoidal data-generating pattern while yielding tight but reliable confidence intervals.


\looseness -1 \textbf{\ours provides accurate predictions. } We perform a comprehensive benchmark study with the environments and baselines introduced in Sec. \ref{sec:exp_setup}. Table \ref{meta_learning_mse} reports RMSE on unseen meta-test tasks. Both MARS-GP and MARS-BNN yield substantial improvements in the RMSE compared to the non-meta-learning baselines and significantly outperforms all other meta-learning baselines in most environments. This shows that \ours can acquire valuable inductive biases from data reliably. We hypothesize that \ours performs substantially better than PACOH-NN, which meta-learns restrictive diagonal Gaussian priors over $\Theta$ since it has much more flexibility in expressing prior knowledge about the data-generating process. In the majority of environments, MARS also outperforms PACOH-GP which meta-learns a GP prior. In contrast to Gaussian marginals, MARS can meta-learn any stochastic process marginal, and, thus has much more flexibility to express inductive bias. 


\looseness -1 \textbf{\ours yields well-calibrated uncertainty estimates. } We hypothesize that by performing meta-learning in the function space, we avoid the pitfalls of NN over-parametrization, which often lead to over-confidence. To investigate the quality of uncertainty estimates, we compute the {\em calibration error}, which measures how much the predicted confidence regions deviate from the actual frequencies of test data in the respective regions. We list the results in Table \ref{meta_learning_ece}\footnote{ Note that we omit MAML since it does not provide uncertainty estimates. }.
While, in most cases, still better than the baselines, the uncertainty estimates \ours-BNN are on average worse than those of \ours-GP. This is not surprising as the MC-dropout uncertainty estimates are typically not as reliable as those of a GP. \ours-GP consistently yields the best-calibrated uncertainty estimates and, for some environments, reduces the calibration error by more than 30 \% compared to the next best baseline.
This provides further evidence for the soundness and efficacy of our function space approach to meta-learning. Finally, the superior calibration performance suggests that the spectral regularization, together with the posterior uncertainty sampling in Sec. \ref{sec:method2}, effectively prevents meta-overfitting and accounts for epistemic uncertainty.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspacecaption
\subsection{Ablation Study}
\vspacecaptionlow
\label{ablation_study_}

\begin{table}[t]
  \centering
  \resizebox{0.95 \textwidth}{!}{
  \begin{tabular}{l|ccccc}
    \toprule
    Estimator     & SwissFEL   & Physionet-GCS  & Physionet-HCT  & Berkeley-Sensor & Argus-Control\\
    \midrule
    \ours-GP & \textbf{0.391} $\pm$ \textbf{0.011} & \textbf{1.471} $\pm$ \textbf{0.083} & \textbf{2.309} $\pm$ \textbf{0.041} & \textbf{0.116} $\pm$ \textbf{0.024} & \textbf{0.013} $\pm$ \textbf{0.001}\\
    SSGE score estimates & 0.449 $\pm$ 0.027 & 3.292 $\pm$ 0.562 & 2.784 $\pm$ 0.257 & 1.105 $\pm$ 0.562 & 0.030 $\pm$ 0.003 \\
    No spectral reg. & 0.420 $\pm$ 0.060 & 2.208 $\pm$ 0.338  & \textbf{2.560} $\pm$ \textbf{0.341} & 1.734 $\pm$ 0.169 & \textbf{0.014} $\pm$ \textbf{0.001} \\
    No GP sampling & 0.471 $\pm$ 0.059 & 2.994 $\pm$  0.363 & 5.995 $\pm$ 1.108 & 1.253 $\pm$ 0.112 & 0.073 $\pm$ 0.003 \\ \bottomrule
  \end{tabular}}
    \vspace{-4pt}
  \caption{Ablation study results for MARS components in terms of the RMSE. \vspace{-6pt}}
  \label{ablation_rmse}
\end{table}

\begin{table}[t]
  \centering
  \resizebox{0.9 \textwidth}{!}{
  \begin{tabular}{l|ccccc}
    \toprule
    Estimator     & SwissFEL   & Physionet-GCS  & Physionet-HCT  & Berkeley-Sensor & Argus-Control\\
    \midrule
    \ours-GP & \textbf{0.035} $\pm$ \textbf{0.002} & 0.263 $\pm$ 0.001 & \textbf{0.136} $\pm$ \textbf{0.007} & \textbf{0.080} $\pm$ \textbf{0.005} & \textbf{0.055} $\pm$ \textbf{0.002} \\
    SSGE score estimates & 0.151 $\pm$ 0.001  & 0.249 $\pm$ 0.002 & 0.246 $\pm$ 0.007 & 0.232 $\pm$ 0.010 & 0.210 $\pm$ 0.011 \\
    No spectral reg. & 0.233 $\pm$ 0.041 & 0.265 $\pm$ 0.012 & 0.244
    $\pm$ 0.009 & 0.192
    $\pm$ 0.018 & 0.187 $\pm$ 0.028 \\
    No GP sampling & 0.204 $\pm$ 0.013 &  \textbf{0.225} $\pm$ \textbf{0.021}  & 0.237 $\pm$ 0.018 & 0.141
 $\pm$ 0.029 & 0.216 $\pm$ 0.066 \\
    \bottomrule
  \end{tabular}}
    \vspace{-4pt}
  \caption{Ablation study results for MARS components in terms of the calibration error. \vspace{-10pt}}
  \label{ablation_ece}
\end{table}


We empirically investigate the algorithm components introduced in Sec. \ref{sec:method2} and provide supporting empirical evidence for our design decisions. 
%
First, we perform a quantitative ablation study where we vary/remove components of our algorithm. We consider \ours-GP with
1) nonparametric score estimator SSGE \citep{ssge} instead of the parametric score network + score matching from Sec. \ref{sec:score_matching_marginals},
2) without spectral regularization, and
3) without GP posterior sampling, i.e., using the GP posterior mean instead of samples for the score matching.
Table \ref{ablation_rmse} and \ref{ablation_ece} report the quantitative results of this ablation experiment. In the following, we discuss the three aspects separately:


\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \vspace{-3pt}
         \includegraphics[width=\linewidth, trim= 0 30 0 0, clip]{iclr2023/images/fig_3_a.pdf}
         \vspace{-13pt}
         \caption{SSGE vs. score network}
         \label{fig:spiky_preds_score1}
     \end{subfigure}
     \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
          \vspace{-3pt}
         \includegraphics[width=\linewidth, trim= 0 30 0 0, clip]{iclr2023/images/fig_3_b.pdf}
         \vspace{-13pt}
         \caption{spectral regularization}
         \label{fig:spiky_preds_score2}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
     \centering
      \vspace{-3pt}
     \includegraphics[width=\linewidth, trim= 0 30 0 0, clip]{iclr2023/images/fig_3_c.pdf}
     \vspace{-13pt}
     \caption{Corresponding density}
     \label{fig:spiky_preds_score3}
    \end{subfigure}
    \vspace{-4pt}
    \caption{(a) Underconfident \ours and overconfident SSGE score predictions on ten samples from a Gaussian. (b) Score estimates of MARS with and without regularization on ten function samples from a zero mean GP with SE kernel. (c) Numerically integrated score predictions corresponding to the scores in (b). Overall, SSGE and MARS w/o regularization overfit and underestimate the variance, whereas spectral normalization biases MARS towards higher entropy. \vspace{-8pt}}
    \label{fig:ablation_study_score_estimates}
        % We fit a non-regularized network and \textsc{\ours} to 10 functional samples from a zero mean GP with an RBF kernel, sampled based on random Fourier features \citep{rff}. $5$-dimensional inputs $x$ are sampled uniformly from $[-7, 7]^5$;
    % the network is given function evaluations with additive Gaussian noise (zero mean, $0.1$ s.d.). For plotting, we uniformly sample inputs and fix functional evaluations to zero of all but one randomly chosen input: we interpolate its $y$-values from the 0.025th until 0.975th percentile. We plot the predictions and the numerically integrated pdf.
\end{figure}

%\looseness -1
\textbf{Parametric score matching outperforms nonparametric score estimation. }
In Sec. \ref{sec:score_matching_marginals} we have introduced a parametric score network which we train with the score matching loss. Alternatively, for each measurement set $\bX$, we could apply the nonparametric score estimator SSGE \citep{ssge} to the function values $\tilde{\rvf}^\bX_1, ..., \tilde{\rvf}^\bX_n$, sampled from the posteriors, and directly use the resulting score estimates during the fSVGD posterior inference in (\ref{eq:fsvgd_updates}). This produces score estimates 'ad-hoc' and does not require us to train an explicit score network. In contrast, our score network is a global function that explicitly considers the measurement set and thus can exploit similarity structure across $\calX$, which SSGE cannot. To SSGE we also cannot simply add inductive bias towards higher entropy as we do through spectral normalization. Overall, the experiment results in Table \ref{ablation_rmse} and \ref{ablation_ece} suggest that instantiating our general approach with SSGE performs worse than \ours. We can also observe this visually in Fig. \ref{fig:spiky_preds_score1}, where we plot the score estimate of \ours and SSGE for a GP marginal where the true score is known. While the \ours score network slightly overestimates the variance of true generative-process marginal, SSGE implicitly underestimates the prior variance, leading to over-confident predictions. 
Finally, Table \ref{fig:MSE_par_vs_nonpar} in Appx. \ref{appx:furtherexperiments} quantitatively shows that the \ours score network provides the most accurate estimates compared to a variety of nonparametric estimators. 


\looseness -1 \textbf{Spectral normalization prevents meta-overfitting. }
In Sec. \ref{sec:regulaization}, we added spectral normalization to our score network. Here, we empirically investigate what happens when we remove the spectral normalization from \ours. Figure \ref{fig:spiky_preds_score2} and \ref{fig:spiky_preds_score3} illustrate how our score network over-fits and under-estimates the true data-generating variance when we do not use spectral regularization. Quantitatively, we observe substantial increases in calibration errors and a consistent worsening of the predictive accuracy. Overall, this highlights the empirical importance of spectral normalization for preventing meta-overfitting and biasing the score estimates toward higher entropy.


\looseness -1 \paragraph{Accounting for epistemic uncertainty of the GP interpolators is crucial.}
In \ours, we interpolate each dataset with a GP or BNN and, when performing score estimation, use samples from the posterior marginals to account for the epistemic uncertainty of the interpolation. Here, we empirically study what happens if we ignore the epistemic uncertainty and take each GP's mean predictions. When doing so, we observe detrimental effects on the RMSE and calibration error in the majority of the environments in Table \ref{ablation_rmse} and \ref{ablation_ece}. This affirms that propagating the epistemic uncertainty of the interpolation into the score estimates is a critical component of \ours.



% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{iclr2023/images/sumpic.png}
%     \caption{We sample 10 functions from the SinusoidSim environment and evaluate each function at five randomly selected inputs outside the $[-2,2]$ range. In the first two plots, the fitted GPs correctly produced wider uncertainty bounds in the $[-2,2]$ range. A naive approach would be to train \ours on mean predictions (or any other interpolation method), yielding the predictions in the second plot. If instead, we train using the GP samples, the network successfully reasons about this uncertainty, as shown on the right plot.}
%     \label{sumpic}
% \end{figure}



==> iclr2023/content/intro.tex <==
\vspacecaption
\section{Introduction}
\vspacecaptionlow
\looseness -1 Using data from related tasks is of key importance for sample efficiency. Meta-learning attempts to extract prior knowledge (i.e., inductive bias) about the unknown data generation process from these related tasks and embed it into the learner so that it generalizes better to new learning tasks \citep{thrun1998, vanschoren2018meta}. Many meta-learning approaches try to amortize or re-learn the entire inference process \citep[e.g.,][]{santoro2016meta, Mishra2018,  garnelo2018neural} or significant parts of it \citep[e.g.,][]{finn2017model, bmaml}. As a result, they require large amounts of meta-training data and are prone to meta-overfitting \citep{qin2018rethink, rothfuss2021pacoh}. 

\looseness -1 The Bayesian framework provides a sound and statistically optimal method for inference by combining prior knowledge about the data-generating process with new empirical evidence in the form of a dataset. 
%Thus, in principle, there is no need for re-learning statistical inference, and we can focus our efforts on meta-learning informative Bayesian priors.
In this work, we adopt the Bayesian framework for inference at the task level and only focus on meta-learning informative Bayesian priors. 
%.  
Previous approaches \citep{mlapmaml, rothfuss2021pacoh} meta-learn Bayesian Neural Network (BNN) prior distributions from a set of related datasets; by meta-learning the prior distribution and applying regularization at the meta-level, they facilitate positive transfer from only a handful of meta-training tasks. However, BNNs lack a parametric family of (meta-)learnable priors over the high-dimensional space of neural network (NN) parameters that is both computationally viable and, simultaneously, flexible enough to account for the over-parametrization of NNs. In practice, both approaches use a Gaussian family of priors with a diagonal covariance matrix, which is too restrictive to accurately match the complex probabilistic structure of the data-generating process.

\looseness -1 To address these shortcomings, we take a new approach to formulating the meta-learning problem and represent prior knowledge in a novel way. We build on recent advances in functional approximate inference for BNNs that perform Bayesian inference in the function space rather than in the parameter space of neural networks  \citep{wang2018stein, sun2019}. When viewing the BNN prior and posterior as stochastic processes, the perfect Bayesian prior is the (true) data-generating stochastic process itself. Hence, we view the meta-training datasets as samples from the meta-data-generating process and interpret meta-learning as empirically estimating the law of this stochastic process. 
More specifically, we meta-learn the {\em score function} of its marginal distributions, which can then directly be used as a source of prior knowledge when performing approximate functional BNN inference on a new target task. %Meta-learning the prior marginal 
% Since scores do not have to integrate to one, 
This ultimately allows us to use flexible neural network models for learning the score and overcome the issues of meta-learning BNN priors in the parameter space.

\looseness -1 In our experiments, we demonstrate that our proposed approach, called {\em Meta-learning via Attention-based Regularised Score estimation (MARS)}, consistently outperforms previous meta-learners in predictive accuracy and yields significant improvements in the quality of uncertainty estimates. Notably, \ours enables positive transfer from only a handful of tasks while maintaining reliable uncertainty estimates. This promises fruitful future applications to domains like molecular biology or medicine, where meta-training data is scarce and reasoning about epistemic uncertainty is crucial.














% \subsection{OLD INTRO:}
% \textit{Meta-learning} attempts to extract prior knowledge (i.e. inductive bias) about the unknown data generation process to improve the learning process. Doing so can provably speed up the learning process, reduce the amount of data required, and boost model performance
% To extract knowledge the meta-data, meta-learning utilizes various optimization strategies. Most common approaches infer neural network (NN) weights that can be quickly adapted to new tasks \citep{maml, maml2, maml3}. However, learning this inductive bias comes with several challenges: \emph{(i)} the obtained measurements might be taken under different circumstances, \emph{(ii)} the available meta-data might be scarce, causing meta-overfitting \citep{metaoverfitting} \emph{(iii)} not all inherent properties of the unknown functional process are represented in the meta-data. For these reasons and more, inferring the weights of a NN does not suffice. Instead of inferring the weights, researchers take one step further and attempt to reason about uncertainty by inferring distributions over the weights \citep{bmaml, pmaml, rothfuss2021pacoh}. This allows for identification and quantification of the aforementioned challenges, as well as provides confidence in the model predictions.

% Uncertainty estimation has, however, been of key interest in Bayesian deep learning (BDL) for a long time. Among several approaches to BDL, Bayesian neural networks (BNNs) \citep{blundell2015weight} have undoubtedly stood out due to their expressivity and predictive capability. Together with the ability to incorporate inductive bias and prior beliefs via the Bayes theorem, BNNs prove especially appealing for uncertainty quantification in meta-learning. Inductive bias and prior beliefs are most commonly represented in the form of a parameterized prior over the BNN weights \citep{amortmaml, bmaml, pmaml}. However, due to its high-dimensionality, this parameterization requires careful hand-crafting and introduces several optimization challenges.


% Recently, BDL community recognized the overparameterization problem \citep{overparam1, overparam2}, causing a significant shift from inferring distributions over the weights, to directly inferring about the stochastic processes induced by BNNs, termed functional BNNs (fBNNs). However, performing Bayesian inference in function-space (rather than weight-space) introduced implementation difficulties which in turn hindered practical applications, including meta-learning ones.


% \subsection{The implementation difficulty of function-BNNs (fBNNs)}

% \begin{figure}[!tbp]
%   \centering
%   \subfloat[SVGD]{\includegraphics[width=0.3\textwidth]{iclr2023/images/intro_plot_SVGD.png}\label{badssgenu}}
%   \hfill
%   \subfloat[GP-fSVGD]{\includegraphics[width=0.3\textwidth]{iclr2023/images/intro_plot_GP.png}\label{goodlaplacet}}
%     \hfill
%   \subfloat[ARSEN]{\includegraphics[width=0.3\textwidth]{iclr2023/images/intro_plot_ARSEN.png}\label{goodlaplacet}}
%   \caption{Comparison of BNN with parameter space prior, fBNN with vanilla GP prior and fBNN with ARSEN}
% \end{figure}

% Maximizing the function-space posterior induced by the fBNN requires a function-space prior $p(f)$ choice. Specifically, one needs to choose between: \emph{(i)} explicit stochastic processes, e.g., Gaussian processes (GPs) \citep{gps} or Student-t processes \citep{shah2014student}, and \emph{(ii)} implicit processes. It can be easily shown that in both cases, information about the functional prior $p(f)$ only enters the training dynamics through $\nabla_{\mathbf{f}} \log p(\mathbf{f})$, i.e., the \textit{prior score}. While explicit processes may be appealing due to their closed-form marginal distributions, explicit-process-fBNNs often lack expressivity and perform poorly in the low-data regime. An example of this is given in Figure \ref{gppriorbnn}. The increase in expressivity and flexibility of implicit processes comes at a cost; the prior score $\nabla_{\mathbf{f}} \log p(\mathbf{f})$ requires statistical estimation. Due to the promising potential of implicit-prior-fBNNs, as demonstrated in Figure \ref{gppriorssge}, we investigate them further.

% Theoretical superiority of implicit-process-fBNNs (to parameter-space BNNs) \citep{DBLP:journals/corr/abs-1903-05779, wang2019function} requires oracle access to infinitely many functions from the underlying stochastic process. In practice, this requirement can be avoided by manually selecting an implicit process whose evaluations can be requested infinitely often, or by using statistically-related data to infer about the implicit process score directly, e.g., by fitting a score estimator to the data.
% The former case requires domain-expert knowledge and presents another difficult hand-crafting task, hence we focus our attention to the latter. 

% Theoretical assumption of access to infinitely many functions from the underlying stochastic process can be avoided in practice by having access to a large enough number of functions which can be evaluated everywhere (or at least in the domain of interest). This is required due to the incapability of score estimation methods to deal with stochastic processes; as every set inputs $x_i$ induces a different conditional distribution $p(y|x)$, score estimation methods cannot reason about samples from other distributions, even if the measurement points were very close, as shown in Figure \ref{closeenough}.

% To the best of our knowledge, the research community has not provided a solution for these challenges and practical applications of fBNNs remain scarce. In this work, we propose \textsc{ARSEN}: an attention-based, regularized score estimation network that provides input-domain interpolation and prevents overfitting in the output-domain. We provide empirical evidence that \textsc{ARSEN} successfully incorporates inductive bias into the fBNNs and show that the overall meta-learning framework achieves state-of-the-art performance across several meta-learning tasks.

% \subsection{Summary of Results}

% We outline the main contributions of our work.
% \begin{itemize}
%     \item We develop a novel neural network architecture that significantly outperforms current score estimation methods. Our method allows for incorporation of fBNN methods into settings with efficient number of calls to the underlying data generation process.  
%     \item We empirically demonstrate that the combination of proposed architecture and loss-regularization successfully prevents meta-overfitting.
%     \item We provide a thorough comparison, showcasing that our meta-learning framework achieves state-of-the-art performance both in terms of predictive accuracy and uncertainty calibration on various datasets.
% \end{itemize}

==> iclr2023/content/method.tex <==
\vspacecaption
\section{Meta-Learning as Score Estimation in the Function Space} 
\vspacecaptionlow
\label{sec:method1}

\vspacesubcaption
\subsection{Problem Statement: Meta-Learning}
\vspacesubcaptionlow
\label{sec:problem_statement}

Meta-learning extracts prior knowledge (i.e., inductive bias) from a set of related learning tasks to accelerate inference on a new and unseen learning task.
%In the context of supervised learning, 
The meta-learner is given $n$ datasets $\calD_{1}, ..., \calD_{n}$, where each dataset $\calD_{i} = (\bX^\calD_i, \by^\calD_i)$ consists of $m_i$ noisy function evaluations $y_{i,t} = f_i(\bx_{i, t}) + \eps$ corresponding to a function $f_i: \calX \mapsto \calY \subseteq \R$ and additive $\sigma$ sub-Gaussian noise $\eps$. In short, we write $\bX^\calD_i = (\bx_{i,1}, ..., \bx_{i,m_i})^\top$ for the matrix of function inputs and $\by^\calD_i = (y_{i,1}, ..., y_{i,m_i})^\top$ for the vector of corresponding observations. 
%
Following previous work \citep[e.g.,][]{baxter2000model, pentina2014pac, rothfuss2021pacoh}, we assume that the functions $f_i \sim \calT$ are sampled i.i.d. from a task distribution $\calT$, which can be thought of as a stochastic process $p(f)$ that governs the random function $f: \calX \mapsto \calY$. 

Our goal is to {\em extract knowledge from the observed datasets, which can then be used as a form of prior for learning a new, unknown target function $f^* \sim \calT$} from a corresponding dataset $\calD^*$. By performing Bayesian inference with a meta-learned prior that is attuned to the task distribution $\calT$, we hope to obtain posterior predictions that generalize better.

\vspacesubcaption
\subsection{Shortcomings of Meta-Learning Priors in the Parameter Space}
\vspacesubcaptionlow
%From a Bayesian perspective, the perfect prior is the probability distribution of the data-generating process itself, i.e., $p(f)$. 

Previous work phrases meta-learning as hierarchical Bayesian problems and tries to meta-learn a prior distribution $p(\theta)$ on the NN weight space that resembles $p(f)$ \citep[e.g.,][]{mlapmaml, rothfuss2021pacoh}. This approach suffers from the following central issues: Due to the over-parameterized nature of neural networks, a large set of parameters $\theta$ correspond to exactly the same mapping $h_\theta(\cdot)$. This makes specifying a good prior distribution $p(\theta)$ typically very difficult. At the same time, there is a lack of sufficiently rich parametric families of distributions over the high-dimensional parameter space $\Theta$ that are also computationally viable. So far, only the very restrictive Gaussian family of priors with diagonal covariance matrices has been employed. As a result, the meta-learned posterior lacks the necessary flexibility to match the complex probabilistic structure of the data-generative process accurately.

\vspacesubcaption
\subsection{ Meta-Learning as Score Estimation on the Data-Generating Process}
\vspacesubcaptionlow
\label{sec:estim_data_gen_proc}

Aiming to address these issues, we acquire prior knowledge in a data-driven manner with a new perspective. We develop a novel approach to meta-learning which hinges upon three key ideas:

First, we view BNN inference in the function space (see Sec.~\ref{sec:background}), i.e., as posterior inference $p(h |\mathbf{X}^{\mathcal{D}}, \mathbf{y}^{\mathcal{D}}) \propto p(\mathbf{y}^{\mathcal{D}} | \mathbf{X}^{\mathcal{D}},h) p(h)$ over neural network mappings $h_\theta: \calX \mapsto \calY$ instead of parameters $\theta$. From this viewpoint, the prior, which is the target of our meta-learning problem, is $p(h)$, a stochastic process on the function space. This alleviates the aforementioned problem of over-parametrization, which arises when considering priors on the parameter space.

Second, we ask ourselves what is a desirable prior: from a Bayesian perspective, the best possible prior is the stochastic process of the task generating distribution $\calT$ itself, i.e., $p(h) = p(f)$. Hence, we would want to meta-learn a prior that matches $p(f)$ as closely as possible. Since the meta-training datasets $\calD_1, ..., \calD_n$ constitute noisy observations of the function draws $f_1, ...., f_n \sim p(f)$, we can use them to estimate the stochastic process marginals $p(\rvf^\bX)$. Crucially, we tractably represent and estimate the stochastic process $p(f)$ through its finite marginals $p(\rvf^\bX)$ in measurement sets $\bX$.

Our third insight is that all popular approximate inference methods for BNNs only use the prior score, i.e., the gradient of the log-prior, and not the prior distribution itself. In addition, parametrizing and estimating the prior score is computationally easier than the prior distribution itself since it does not have to integrate to 1, allowing for much more flexible neural network representations. For this reason, our meta-learning approach directly forms an estimate of the scores $s(\rvf^{\bX}, \bX) = \nabla_{\rvf^\bX} \ln p(\rvf^\bX)$ of the data-generating process marginals. \looseness -1

In summary, our high-level approach is to {\em meta-learn / estimate the prior score $\nabla_{\rvh^\bX} \ln p(\rvh^\bX)$ that matches data-generating stochastic process from meta-training data $\calD_1, ..., \calD_n$}. At meta-test time, the meta-learned prior marginals are used in the approximate functional BNN inference on a target dataset $\calD^*$ to infuse the acquired prior knowledge into the posterior predictions. 
In the following section, we discuss in more detail how to implement this general approach as a concrete, computationally feasible algorithm with strong empirical performance.


% In particular, our approach is based on the following insights: 
% \begin{enumerate}
%     \item Phrasing the Bayesian inference with NNs in the function space alleviates the aforementioned problem of over-parametrization.
%     \item From a Bayesian perspective, the best possible prior is the probability distribution of the data-generating process itself, i.e., $p(h) = p(f)$.
%     \item All popular approximate inference methods for BNNs only use the prior score, i.e., the gradient of the log-prior, and not the prior distribution itself \citep[e.g.][]{welling2011bayesian, blundell2015weight, Liu2016}. Parametrizing and estimating the prior score is easier than the prior distribution since it does not have to integrate to 1, thus allowing for much more flexible neural network representations.
% \end{enumerate}

% Our proposed meta-learning method builds on the recent advances in functional space approximate inference for BNNs (see Section \ref{sec:fbnns}). Existing fBNNS approaches presume a stochastic process prior as exogenously given \citep{wang2019function, sun2019}. Additionally, they require oracle access to arbitrarily many sampled functions as well as the ability to evaluate them in arbitrary input values (i.e., measurement sets). This allows them repeatedly draw samples from the finite marginals $p(\rvh^\bX)$ in random measurement sets $\bX$ and use SSGE \citep{ssge} or Gaussian approximations to estimate the prior score $\nabla_{\rvh^\bX} \ln p(\rvh^\bX)$.

% In contrast, we aim to {\em meta-learn / estimate the prior score $\nabla_{\rvh^\bX} \ln p(\rvh^\bX)$ that corresponds to the task distribution $\calT$ (i.e., the data-generating stochastic process) based on the meta-training data $\calD_1, ..., \calD_n$}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspacecaption
\section{The MARS meta-learning algorithm}
\vspacecaptionlow
\label{sec:method2}

In Section \ref{sec:method1}, we have motivated and sketched the idea of meta-learning via score estimation of the data-generating process marginals. We now discuss particular challenges and outline the design choices for translating this idea into a practical meta-learning algorithm. 

Score estimation of stochastic process marginals has previously been used in the context of existing functional BNN approaches \citep{wang2019function, sun2019}. However, they presume a known stochastic process prior with oracle access to arbitrarily many sampled functions that can be evaluated in arbitrary locations of the domain $\calX$. Compared to such a stochastic process prior with oracle access, we face two key challenges which make the score estimation problem much harder: 
\begin{enumerate}
    \item We only have access to a finite number of datasets $\{\calD_i\}_{i=1}^n$,  each corresponding to one function $f_i$ drawn from the data-generating stochastic process. This means, we have so estimate the marginal scores $\nabla_{\rvh^\bX} \ln p(\rvh^\bX)$ from only $n$ function samples without over-fitting. \looseness-1
    \item Per function $f_i$, we only have a limited number of $m_i$ noisy function evaluations $\by^\calD_i$ in input locations $\bX^\calD_i$ which are given to us exogenously, and we have no control over them. However, to perform score estimation for the marginal $p(\rvh^\bX)$ distributions, for each function, we need a vector of function values $\mathbf{f}_i^\bX$ evaluated in the measurements points $\bX$.
\end{enumerate}

In the following subsections, we present our approach to estimating the stochastic prior scores and discuss how to solve these challenges. In addition, we discuss how to perform functional approximate BNN inference with the meta-learned score estimates. %Finally, we compare our approach to several state-of-the-art nonparametric score estimators and provide the findings in Appendix \ref{param_vs_nonparam}.

\vspacecaption
\subsection{Parametric Score Matching for Stochastic Process Marginals}
\vspacecaptionlow
\label{sec:score_matching_marginals}


Performing functional approximate inference with fSVGD updates as in (\ref{eq:fsvgd_updates}) requires estimation of the prior marginal scores $ \nabla_{\rvh^\bX} \ln p(\rvh^\bX)$ for arbitrary measurement sets $\bX$. A key property of stochastic process marginal scores is their permutation equivariance: if we permute the order of the points in the measurement set, the rows of the score permute in the same manner. Similarly, the measurement sets can be of different sizes, implying score vectors/matrices of different dimensionalities.\looseness-1

\looseness -1 Aiming to embed these properties into a parametric model of the prior marginal scores, we use a transformer encoder architecture \citep{vaswani2017attention}, that takes as an input a measurement set $\bX \in \R^{\text{dim}(\calX) \times k}$ of $k$ points and corresponding query function values $\rvh^\bX \in \R^{\text{dim}(\calY) \times k}$ and performs attention over the second dimension, i.e., the $k$ columns corresponding to measurement points. Our score network model is denoted as $\rvs_\phi(\rvh^\bX, \bX)$ with trainable parameters $\phi$ and outputs an estimate of the score, i.e., $\rvs_\phi(\rvh^\bX, \bX) \mapsto \tilde{\nabla}_{\rvh^\bX} p(\rvh^\bX)$, a matrix of the same size as the query function values.
%$\rvs_\phi: \R^{\text{dim}(\calX) \times k} \times \R^{\text{dim}(\calY) \times k} \mapsto \R^{\text{dim}(\calY) \times k}$
The model is permutation equivariant w.r.t.~the columns corresponding to measurement points and supports inputs/outputs for varying measurement set sizes $k$. We schematically illustrate the score network architecture in Figure~\ref{fig:network_architecture} and provide details in Appendix \ref{appx:score_estimation_details}.

We train the score network with a modified version of the score matching loss \citep{hyvarinen2005estimation, slicedscorematching}. This loss minimizes the Fisher divergence between the data-generating process marginals and our score network, based on samples $\rvf^\bX_1, ..., \rvf^\bX_n$ from the data-generating process marginals. In contrast to the standard score matching loss, our modified loss takes the dependence of stochastic process marginals on their measurement sets into account. It uses an expectation over randomly sampled measurement sets, similar to the functional approximate inference in Section \ref{sec:background}.
\begin{equation} \label{eq:score_matching_loss}
    \calL(\phi) := \E_\bX \left[ \frac{1}{n} \sum_{i=1}^n  \left( \text{tr}(\nabla_{\rvf_i^\bX} \rvs_\phi(\rvf_i^\bX, \bX)) + \frac{1}{2} || \rvs_\phi(\rvf_i^\bX, \bX) ||_2^2 \right) \right]
\end{equation}
As noted previously, our meta-training data only provides noisy function evaluations for a limited, exogenously given, set of input locations per task $f_i$. The input locations $\bX^\calD_i$ per task might even differ in number and be non-overlapping. Thus, we do not have access to the function values $\rvf^\bX_1, ..., \rvf^\bX_n$ for arbitrary measurement sets $\bX$ which we require for our score matching loss in (\ref{eq:score_matching_loss}). In the following section, we discuss how to resolve this problem.

\vspacecaption
\subsection{Interpolating the Datasets across \texorpdfstring{$\calX$}{X}}
\vspacecaptionlow
\label{sec:method_interpolating}
In our meta-learning setup (see Section \ref{sec:problem_statement}), we only receive noisy function evaluations $\mathbf{y}^\calD_i$ in $m_i$ locations $\bX^\calD_i$ for each meta-training task. However, to minimize the score matching loss in (\ref{eq:score_matching_loss}), we need the corresponding function values in arbitrary measurement locations in the domain $\calX$.

Hence, we interpolate each dataset $\calD_i$ by a regression model. Importantly, the regression model should be able to quantify the epistemic uncertainty that stems from having observations at only a finite subset of points $\bX^\calD_i \subset \calX$. While a range of method could be used, we employ a Gaussian Process (GP) with Matérn$-5/2$ kernel or a Bayesian neural network (BNN) based on Monte Carlo dropout \citep{gal2016dropout} for this purpose.
We fit the respective Bayesian model independently on each dataset $\calD_i$ which gives us a posterior $p(\rvf_i^\bX| \bX,  \bX^\calD_i, \mathbf{y}^\calD_i)$ over function values $\rvf_i^\bX$ for arbitrary measurement sets $\bX$. In Appx. \ref{appx:fitting_the_gps} we provide more details on how we fit each model.

While we could simply use posterior mean values for computing the score matching loss in \ref{eq:score_matching_loss}, this would not reflect the epistemic interpolation uncertainty.
Instead, for each task, we sample function values $\tilde{\rvf}_i^\bX \sim p(\rvf_i^\bX| \bX, \bX^\calD_i, \mathbf{y}^\calD_i)$ from the corresponding posterior and use them as an input to the score matching loss in (\ref{eq:score_matching_loss}). Correspondingly, the score matching loss modifies to
%
\begin{equation} \label{eq:score_matching_loss_post_sampling}
    \tilde{\calL}(\phi) := \E_\bX \left[ \frac{1}{n} \sum_{i=1}^n \E_{p(\tilde{\rvf}_i^\bX| \bX, \bX^\calD_i, \mathbf{y}^\calD_i)} \left[ \text{tr}(\nabla_{\tilde{\rvf}_i^\bX} \rvs_\phi(\tilde{\rvf}_i^\bX, \bX)) + \frac{1}{2} || \rvs_\phi(\tilde{\rvf}_i^\bX, \bX) ||_2^2 \right] \right] \;.
\end{equation}
%
\looseness=-1 The further a measurement point $x$ is away from the closest point in $\bX^\calD_i$, the higher is the (epistemic) uncertainty of the corresponding function value $f_i(x)$. By sampling from the posterior, in expectation, the loss in (\ref{eq:score_matching_loss_post_sampling}) effectively propagates the interpolation uncertainty into the score matching procedure, preventing over-confident score estimates for areas of the domain $\calX$ with scarce data. This is illustrated in Appx. \ref{appx:furtherexperiments}, Figure \ref{fig:GP_with_and_without}.

\vspacecaption
\subsection{Preventing Meta-Overfitting of the Prior Score Network}
\vspacecaptionlow
\label{sec:regulaization}
\looseness=-1 The final challenge we need to address is over-fitting to the meta-training tasks \citep{yin2020meta, rothfuss2021pacoh}. As we only have meta-training data $\{\calD_i\}_{i=1}^n$, corresponding to $n$ functions $f_i$ drawn from the data-generating stochastic process, i.e., we only have $n$ samples for estimation of marginal scores $\nabla_{\rvh^\bX} \ln p(\rvh^\bX)$, making us prone to overfitting the prior score network. If we performed functional BNN inference with such an overfitted score estimate, the BNN's posterior predictions are likely to be over-confident and too biased towards the functions seen during meta-training.

\looseness=-1 To counteract the tendency to overfit, we regularize the score network via spectral normalization \citep{spectralnormalization} of the linear layers in the transformer encoder blocks. Spectral normalization controls the Lipschitz constant of the neural network layers by dividing their weight matrix $\mathbf{W}$ by its spectral norm $||\mathbf{W}||$, i.e., re-parametrizing the weights as $\tilde{\mathbf{W}} := \mathbf{W} / ||\mathbf{W}||$. Hence, by applying spectral normalization, we bias our score network towards smoother score estimates corresponding to marginal distributions $p(\rvh^\bX)$ with higher entropy. Empirically we find that spectral normalization effectively combats meta-overfitting and prevents the estimated prior score from inducing over-confident posterior predictions when employed in functional BNNs. In our experiments, we examined several other regularization methods, e.g., gradient penalties \citep{gradientpenalty} or a spectral regularization penalty in the loss, but found spectral normalization to work the best.

% \subsection{Approximate Functional BNN Inference}
% \label{sec:fbnns}
% To tractably perform approximate posterior inference in the function space, we use functional Stein Variational Gradient Descent (fSVGD) \citet{wang2019function}. 
% %Similarly, the functional variational inference could be employed \citep{sun2019} but tends to perform worse in practice.
% %
% The fSVGD approach approximates the posterior by a set of $L$ NN parameter particles $\{ \theta_1, ..., \theta_L \}$. To optimize the particles in order to approximate the posterior well, fSVGD iteratively re-samples measurement sets $\bX$, computing SVGD \citep{Liu2016} updates in the function space and projecting them back into the parameter space.
% %
% Consistently with our functional approach to meta-learning, it uses the posterior score in function space 
% $\nabla_{\rvh^\bX} \ln p(\rvh^\bX |\mathbf{X}, \mathbf{y}^{\mathcal{D}})  = \nabla_{\rvh^\bX} \ln p(\mathbf{y}^{\mathcal{D}} | \rvh^{\bX^{\mathcal{D}}}) + \nabla_{\rvh^\bX} \ln p(\rvh^{\bX}).$ Formally, the particle updates are computed as 
% %
% \begin{equation} \label{eq:fsvgd_updates}
%     \theta^l \leftarrow \theta^l - \gamma  \left( \nabla_{\theta^l} \rvh_{\theta^l}^\bX \right)^\top  \bigg( \underbrace{\frac{1}{L} \sum_{i=1}^L \bK_{li} \nabla_{\rvh_{\theta^i}^\bX} \ln p(\rvh_{\theta^l}^\bX |\mathbf{X}, \mathbf{y}^{\mathcal{D}}) + \nabla_{\rvh_{\theta^l}^\bX} \bK_{li}}_{\text{SVGD update in the function space}} \bigg) ~, \quad \forall l = 1, ..., L~ \;,
% \end{equation}
% where $K = [k(\rvh_{\theta^l}^\bX, \rvh_{\theta^i}^\bX)]_{li}$ is the kernel matrix between the function values in the measurement points based on a positive semi-definite kernel function $k(\cdot, \cdot)$. 
% When we perform posterior inference with the meta-learned score network, we simply replace the hand-defined prior score $\nabla_{\rvh^\bX} \ln p(\rvh^{\bX})$ with the predictions meta-learned score network $s(\rvh_{\theta^l}^\bX, \bX)$.




% propose to construct random measurement sets $\bX:=[\bX^\calD_{s}, \bX^M]$ by selecting a random subset $\bX^\calD_{s}$ of the training inputs $\bX^\calD$ as well as random points $\bX^M \overset{iid} {\sim} \nu$ sampled independently from a distribution $\nu$ that is supported on $\calX$. The corresponding posterior marginal score follows as

% %
% \begin{equation} \label{eq:functional_post_score}
%   \nabla_{\rvh^\bX} \ln p(\rvh^\bX |\mathbf{X}, \mathbf{y}^{\mathcal{D}})  = \nabla_{\rvh^\bX} \ln p(\mathbf{y}^{\mathcal{D}} | \rvh^{\bX^{\mathcal{D}}}) + \nabla_{\rvh^\bX} \ln p(\rvh^{\bX}) \;.
% \end{equation}
% %
% In this paper, we work with particle approximations of the BNN posterior, where the BNN posterior is approximated by a set of $L$ parameter particles $\{ \theta_1, ..., \theta_L \}$. \citep{wang2019function} propose a functional Stein Variational Gradient Descent (fSVGD) \citep{Liu2016} which iteratively re-samples measurement sets $\bX$, computing SVGD updates in the function space and projecting them back into the parameter space:
% %
% \begin{equation} \label{eq:fsvgd_updates}
%     \theta^l \leftarrow \theta^l - \gamma  \left( \nabla_{\theta^l} \rvh_{\theta^l}^\bX \right)^\top  \bigg( \underbrace{\frac{1}{L} \sum_{i=1}^L \bK_{li} \nabla_{\rvh_{\theta^i}^\bX} \ln p(\rvh_{\theta^l}^\bX |\mathbf{X}, \mathbf{y}^{\mathcal{D}}) + \nabla_{\rvh_{\theta^l}^\bX} \bK_{li}}_{\text{SVGD update in the function space}} \bigg) ~, \quad \forall l = 1, ..., L~.
% \end{equation}
% Here, $K = [k(\rvh_{\theta^l}^\bX, \rvh_{\theta^i}^\bX)]_{li}$ is the kernel matrix between the function values in the measurement points based on a positive semi-definite kernel function $k(\cdot, \cdot)$. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspacecaption
\subsection{The full \ours algorithm}
\vspacecaptionlow

\begin{algorithm}[t]
\begin{algorithmic}
\STATE \textbf{Input:} datasets $\calD_1, ..., \calD_n$, measurement point distribution $\nu$, step size $\eta$
\STATE Initialize score network parameters $\phi$
% \STATE Determine GP kernel lengthscale via CV-gridsearch
\FOR{$i=1,...,n$}
    \STATE fit GP or BNN on $\calD_i$, obtain posterior $p(f_i| \bX^\calD_i, \mathbf{y}^\calD_i)$
\ENDFOR
\WHILE{ not converged}
     \STATE $\bX \overset{iid}{\sim} \nu$ \hfill // sample measurement set
 	\FOR{$i=1,...,n$}
 	    \STATE $\tilde{\rvf}^\bX_i \sim p(\rvf_i^\bX| \bX, \bX^\calD_i, \mathbf{y}^\calD_i)$\hfill // sample function values from posterior marginal
     \ENDFOR
     \STATE $\hat{\calL}(\phi) \leftarrow \frac{1}{n} \sum_{i=1}^n \left( \text{tr}(\nabla_{\tilde{\rvf}_i^\bX} \rvs_\phi(\tilde{\rvf}_i^\bX, \bX)) + \frac{1}{2} || \rvs_\phi(\tilde{\rvf}_i^\bX, \bX) ||_2^2  \right) $ \hfill // score matching loss
	\STATE $\phi \leftarrow \phi + \eta \nabla_\phi \hat{\calL}(\phi)$ \hfill // score network gradient update
\ENDWHILE
\STATE \textbf{Output:} trained score network $\rvs_\phi$
\end{algorithmic}
\caption{\ours: Meta-Learning the Data-Generating Process Score}
\label{algo:score_meta_learning}
\end{algorithm}



%Finally, we summarize the developed approach for equipping BNNs with useful prior knowledge from related data sources in its entirety. 
We now summarize our meta-learning algorithm \ours. It consists of two stages:

\textbf{Stage 1: Meta-Learning the Prior Score Network.}
\looseness -1 After initializing the parameters of the score network, we fit a GP or BNN to each of the $n$ meta-training datasets $\calD_i$. Then, we train the score network by stochastic gradient descent on the modified score matching loss $\tilde{\mathcal{L}}(\phi)$ in (\ref{eq:score_matching_loss_post_sampling}). 
In each iteration, we first sample a measurement set $\bX$ i.i.d.~from the measurement distribution $\nu = \calU(\tilde{\calX})$, chosen as uniform distribution over the hypercube $\tilde{\calX} \subseteq \calX$ conservatively covering the data
%\footnote{We increase the magnitude of each dimension of the hypercube end points by 20\%.}
in $\calX$. Based on the measurement set, we sample a vector of functions values $\tilde{\rvf}^\bX_i$ from the corresponding GP or BNN posterior marginals $p(\rvf_i^\bX| \bX, \bX^\calD_i, \mathbf{y}^\calD_i), i=1, ..., n$.
Based on these samples, we form an empirical estimate $\hat{\calL}(\phi)$ of the score matching loss and perform a gradient update step on the score network parameters $\phi$. This is repeated till convergence and summarized in Alg. \ref{algo:score_meta_learning}. Depending on whether we use a GP or BNN as interpolator, we refer to our method as \ours-GP or \ours-BNN.

\textbf{Stage 2: Functional BNN Inference with the Prior Score Network.}
When concerned with a target learning task with a training dataset $\calD^*= ( \bX_*^\calD, \mathbf{y}_*^\calD)$, we can infuse the meta-learned inductive bias into the BNN inference by using the prior score network $\rvs_\phi$ from Stage 1 for the approximate inference.
In particular, we can either perform functional VI \citep{sun2019} or fSVGD \citep{wang2019function}, using the score network $\rvs_\phi(\rvh^\bX, \bX)$ 
predictions as swap-in replacement for the marginal scores $\nabla_{\rvh^\bX} \ln p(\rvh^{\bX})$ of a user-specified stochastic process prior. In our experiments, we use fSVGD (see Section \ref{sec:background}) as functional approximate inference method. The resulting fSVGD BNN inference procedure with our meta-learned priors score network is summarized in Alg. \ref{algo:fsvgd} in Appx. \ref{appx:implementation_details}.



% In order to tackle overfitting, we gather inspiration from GAN stabilization techniques. More specifically, we consider: \emph{(i)} gradient penalties \citep{gradientpenalty}, where gradient evaluations of points uniformly sampled on a linear interpolation between the data are added as a soft penalty and \emph{(ii)} spectrally normalizing the network's linear layers \citep{spectralnormalization}. We also experiment with the following soft penalties: \emph{(iii)} sum of spectral norms of linear layers, and \emph{(iv)} adding the RKHS norm w.r.t. a curl-free kernel.\footnote{Note that every gradient function has a curl-free kernel; therefore, the network should have a finite RKHS norm w.r.t. a curl-free kernel.} 



% In standard Bayesian inference, we exogenously presume an -- often carefully {\em manually designed} -- prior distribution $P(h)$ over learning hypotheses $h: \calX \mapsto \calY, h \in \calH$ and combine it with empirical data to form a posterior $Q(h)=P(h|\calD)$. In contrast, in meta-learning, we endogenously infer the prior $P(h)$ in a {\em data-driven} manner by using the provided meta-training data.




% \subsection{OLD: Motivation}

% Consider the following supervised learning setting. We are given a dataset $\mathcal{D}^*=\left(\mathbf{X}_i^{\mathcal{D^*}}, \mathbf{y}_i^{\mathcal{D^*}}\right)$ that consists of $n^*$ noisy function evaluations $y_{i}=f^*\left(\mathbf{x}_{i}\right)+\epsilon_i$  corresponding to the unknown function of interest $f^*: \mathcal{X} \mapsto \mathcal{Y}$ and additive noise $\epsilon_i$.  Standard Bayesian inference methods allow to incorporate domain knowledge about $f$ in the form of a prior distribution $P(f)$ over learning hypotheses $f: \mathcal{X} \mapsto \mathcal{Y}, h \in \mathcal{H}$, for some hypothesis space $\mathcal{H}$. The prior distribution, together with the observed data  $\mathcal{D}^*$, is then used to perform posterior inference about $f$. 

% In contrast, meta-learning provides a framework that eases the inference problem by assuming access to $n$ datasets $\mathcal{D}_{1, T_1}, \ldots, \mathcal{D}_{n, T_n}$, statistically related to $\mathcal{D}^*$. The available datasets form the \textit{meta-data} and allow to reason about the underlying stochastic process in a data-driven manner. Each dataset $\mathcal{D}_{i, T_i}=\left(\mathbf{X}_i^{\mathcal{D}}, \mathbf{y}_i^{\mathcal{D}}\right)$ consists of $T_i$ noisy function evaluations $y_{i, t}=f_i\left(\mathbf{x}_{i, t}\right)+\epsilon$. Here, we denote the matrix of function inputs by $\mathbf{X}_i^{\mathcal{D}}=\left(\mathbf{x}_{i, 1}, \ldots, \mathbf{x}_{i, T_i}\right)^{\top}$ and vector containing the corresponding observations by $\mathbf{y}_i^{\mathcal{D}}=\left(y_{i, 1}, \ldots, y_{i, T_i}\right)^{\top}$. Meta-learning views functions $f_i \sim \mathcal{T}$ as sampled from the model distribution $\mathcal{T}$, also termed \textit{task} distribution. However, $\mathcal{T}$ can also be viewed as a stochastic process governing the random functions $f_i: \mathcal{X} \mapsto \mathcal{Y}$. This viewpoint allows us to draw a connection between BDL (more specifically, fBNNs) and meta-learning: we now have access to samples from the underlying stochastic process $\mathcal{T}$ and can use the meta-data directly to reason about $P(f)$.

% In order to unite the two, we split the problem in four steps:
% \begin{enumerate}
%     \item we choose between parametric and nonparametric score estimators
%     \item we enhance the choosen estimator to learn scores of stochastic process marginal distributions
%     \item we tackle meta-overfitting both in the input and output domain
%     \item we incorporate the two into a fBNN-based meta-learning framework
% \end{enumerate}

% \begin{figure}[!tbp]
%   \centering
%   \subfloat[Flower one.]{\includegraphics[width=0.5\textwidth]{iclr2023/images/firstbad.png}\label{gppriorbnn}}
%   \hfill
%   \subfloat[Flower two.]{\includegraphics[width=0.5\textwidth]{iclr2023/images/firstgood.png}\label{gppriorssge}}
%   \caption{Both figures show fBNN predictions trained using only two data points. In Figure \ref{gppriorbnn}, fBNN is trained with a GP prior, which is fitted on the meta-data using cross-validation. Across various kernels (including periodic ones), the observed performance was poor as the GP attributed the sinusoidal oscillations to noise. Figure \ref{gppriorssge} presents the same fBNN, trained using SinusoidSim (see Appendix \ref{sinusoidsim}) as the data generating process. This shows the remarkable potential of the approach: using only two input points and the true, but noised functional prior data, fBNN is able to learn the true mean function far from the training data and yields satisfactory uncertainty estimates.}
% \end{figure}

==> iclr2023/content/related_work.tex <==
\vspacecaption
\section{Related Work}
\vspacecaptionlow

\textbf{Meta-Learning. }
Common approaches in meta-learning amortize the entire inference process \citep{santoro2016meta, Mishra2018, amortmaml, garnelo2018neural}, learn a good neural network initialization \citep{finn2017model, rothfuss2019promp, nichol2018firstorder, kim2018bayesian} or a shared embedding space \citep{baxter2000model, vinyals2016matching, snell2017prototypical}. Although these approaches can meta-learn complex inference patterns, they require a large amount of meta-training data and often perform poorly in settings where data is scarce.
Another line of work uses a hierarchical Bayesian approach to meta-learn priors over the NN parameters \citep{pentina2014pac, mlapmaml, rothfuss2021pacoh}. Such methods perform much better on small data. However, they suffer from the lack of expressive families of priors for the high-dimensional and complex parameter space of NNs, making too restrictive assumptions to represent complex inductive biases. Our approach overcomes these issues by viewing the problem in the function space and directly learning the score, which can easily be represented by a NN instead of a prior distribution. Also related to our stochastic process approach are methods that meta-learn Gaussian Process (GP) priors \citep{fortuin2019deep, rothfuss2021fpacoh, rothfuss2022_safe}. However, the GP assumption is quite limiting, while \ours can, in principle, match the marginals of any data-generating process.

\looseness -1 \textbf{Score estimation. } We use score estimation as a central element of our meta-learning method. In particular, we use a parametric approach to score matching and employ an extended version of the score matching objective of \citet{hyvarinen2005estimation}. For high-dimensional problems, \citet{slicedscorematching, slicedscorematching2} propose randomly sliced variations of the score matching loss.
Alternatively, there is a body of work on nonparametric score estimation \citep{kef, stein, ssge, numethod, nonparametric}. Among those, the Spectral Stein Gradient Estimator \citep{ssge} has been used for estimating the stochastic process marginals for functional BNN inference in a setting where the stochastic prior is user-defined and allows for generating arbitrarily many samples \citep{sun2019}.
Such estimators make it much harder to add explicit dependence on the measurement sets and prevent meta-overfitting via regularization, making them less suited to our problem setting.

% \subsection{OLD PARAGRAPHS FOR REUSE}
% \paragraph{Nonparametric score estimation.}
% There is a plethora of nonparametric score estimation methods; KEF \citep{kef} minimizes a regularized version of the score matching loss between the data score and score of kernel exponential families. NKEF  \citep{nkef} relies on the Nyström method to accelerate KEF by minimizing the loss in a low-dimensional subspace rather than the whole RKHS. \citet{stein} utilize the generalized Stein's identity to propose the Stein estimator, and \citet{ssge} propose Spectral Stein Gradient Estimator (SSGE) by expanding the score function in terms of the spectral eigenbasis. Together with iterative methods ($\nu$-method and Landweber iteration \citep{numethod}), these can be naturally unified through a regularized, nonparametric regression framework \citep{nonparametric}. However, nonparametric estimators present two problems: none of the estimators provide a principled way to reason about stochastic process scores, and in the low-data regime, they result in scores of overconfident distributions, non-smooth distributions.

% \paragraph{Score matching and parametric estimators.} Parametric objectives, as they are expectations, require Monte Carlo estimation and rely heavily on an abundance of data in order to result in solid performance. These objectives have seen large popularity in the field of GANs \citep{gans} where the data assumption is commonly satisfied. Furthermore, due to the high dimensionality of the input/output domain, the subsequent research on the objectives mainly focused on the low-dimensional approximations \citep{slicedscorematching, slicedscorematching2}. However, regularization in the low-data regime remains poorly understood. 

% \paragraph{Probabilistic Model-Agnostic meta-learning methods.} Following MAML, many authors proposed probabilistic model-agnostic alternatives in order to capture predictive uncertainty. In Bayesian-MAML, \citet{bmaml} propose performing meta-learning through a Bayesian ensemble method. Equipped with SVGD, they build on MAML using a probabilistic framework with a modified MAML meta-update loss. In Probabilistic-MAML (PLATIPUS), \citet{pmaml} propose optimizing model parameters with respect to a variational lower bound on the likelihood for the meta-training tasks. This allows learning the variance of the model parameters, whose number scales linearly with the number of model weights. Albeit simple, the variance estimator does not depend on the meta-data and often yields poor uncertainty estimates. 


% \paragraph{PAC-Bayes meta-learning methods.} A few meta-learning methods find inspiration in PAC-Bayes theory; \citet{mlapmaml} propose incorporating prior knowledge by adjusting a learned prior based on the tasks encountered. In particular, they develop a gradient-based algorithm by minimizing PAC-Bayes generalization bounds. However, rather than learning to solve tasks sequentially, their method does so in parallel. Moreover, their framework assumes a bounded loss function and often results in high-variance gradients. \citet{rothfuss2021pacoh} propose a similar framework by developing a class of PAC-optimal meta-learning algorithms and relaxing the previous framework by allowing for unbounded loss functions, as well as achieving positive transfer. 


% \paragraph{Other probabilistic meta-learning methods.} Probabilistic meta-learning methods also employ GPs, BNNs, or Variational Implicit Processes. \citet{vgpmaml} present Variational Meta-Gaussian Processes, using GPs to learn a Gaussian latent variable distribution which is used as a NN input to predict the labels. \citet{amortmaml} propose Amortized Bayesian meta-learning, which learns a prior distribution over weights by amortizing hierarchical variational inference across tasks. Their method also allows for competitive performance but is restricted to less expressive priors (and therefore posteriors) due to the high-dimensional parameterization problem of BNNs.

==> iclr2023/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm,amssymb}

\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}

\newtheorem{theoremA}{Theorem}
\renewcommand{\thetheoremA}{A\arabic{theoremA}}

\newtheorem{lemmaA}{Lemma}
\renewcommand{\thelemmaA}{A\arabic{lemmaA}}
\newtheorem{definition}{Definition}
\newtheorem{remark}{Remark}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak



\newcommand{\rom}[1]
    {\text{\MakeUppercase{\romannumeral #1}}}


% For commenting the draft:
%\usepackage{lineno}
%\linenumbers


%\usepackage[letterpaper, total={6in, 9in}]{geometry}

%\usepackage[square,sort,comma,numbers]{natbib}
%\usepackage{natbib}

%Math commands

\newcommand{\bX}{\mathbf{X}}
\newcommand{\bh}{\mathbf{h}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\obs}[1]{#1^o}
\newcommand{\miss}[1]{#1^m}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bLamb}{\mathbf{\Lambda}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\GP}{\mathcal{GP}}
\newcommand{\bigO}{\mathcal{O}}
\newcommand{\loss}{\mathcal{L}}
\newcommand{\normal}{\mathcal{N}}
\newcommand{\given}{\, \vert \,}

\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}

\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}


\newcommand{\expect}[2]{\mathbb{E}_{#1} \; #2}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bfP}{\mathbf{P}}
\newcommand{\bfTheta}{\mathbf{\Theta}}
\newcommand{\Rhat}{\hat{R}}



\renewcommand{\overline}{\tilde}

%\renewcommand\Affilfont{\footnotesize}


\newcommand{\fix}{\marginpar{FIX}}
\newcommand{\new}{\marginpar{NEW}}

\newcommand{\beginsupplement}{%
        \setcounter{table}{0}
        \renewcommand{\thetable}{S\arabic{table}}%
        \setcounter{figure}{0}
        \renewcommand{\thefigure}{S\arabic{figure}}%
     }
 
\newcommand{\addcitation}{{\color{red} \textbf{[ADD CITATION]} \xspace}}

